Deep Level-set Method for Stefan Problems

We propose a level-set approach to characterize the region occupied by the solid in Stefan problems with and without surface tension, based on their recent probabilistic reformulation. The level-set function is parameterized by a feed-forward neural network, whose parameters are trained using the probabilistic formulation of the Stefan growth condition. The algorithm can handle Stefan problems where the liquid is supercooled and can capture surface tension effects through the simulation of particles along the moving boundary together with an efficient approximation of the mean curvature. We demonstrate the effectiveness of the method on a variety of examples with and without radial symmetry.

==> Intro.tex <==
\section{Introduction}\label{sec:intro}

The Stefan problem \cite{Stefan1,Stefan2,Stefan3,Stefan4} is central in partial differential equations entailing free boundaries. It aims to represent the evolution of temperature in a solid and liquid region separated by a moving interface. Despite its simple description, the Stefan problem still possesses many open questions to this day.  %on the existence,  uniqueness, and regularity of solutions remain open to this day. 
Nevertheless, there has been some recent progress;   \cite{Figalli}  characterize  the singular set of the free boundary; \cite{DNS,MishaScaling,MishaRadialTension} propose the notion of  \textit{probabilistic} solutions aiming to reconcile the existence and uniqueness of solutions.  Indeed, weak solutions to the Stefan problem are typically non-unique, while strong solutions may fail to exist. In fact,   \citet{MishaScaling} shows for  one-phase Stefan problems  that probabilistic solutions lie precisely between weak and strong solutions.  % %and \textit{physical} solutions, which are compared to \textit{minimal} solutions in \cite{CRS}. 
To gain insight, we now summarize the main characteristics of a probabilistic solution. 
First, it satisfies a growth condition relating the change in volume of the solid  (denoted by $\Gamma_t$) to the proportion of absorbed particles in either phase, namely 
\begin{equation*}\label{eq:probaCond2}
\underbrace{|\blue{\Gamma_{0}}| -  |\blue{\Gamma_t}  |}_{\text{Volume change of the solid}}
   = \; \underbrace{\eta\Pb(\tau^1 \le t) - \Pb(  \tau^2 \le t)}_{\text{Absorbed liquid $\&$ solid particles}},   %\tau_{\text{\tiny solid}}_{ \text{\tiny liquid}}
\end{equation*}\\[-1em]
where $\tau^1$ (resp. $\tau^2$)  denotes the hitting time of the moving front $\partial \Gamma = (\partial \Gamma_t)_{t \in [0,T]}$ for particles in the liquid (resp. solid). 
The binary parameter $\eta$ captures the effect of particles in the liquid when the latter  has a nonnegative temperature ($\eta = 1$) or is \textit{supercooled} ($\eta = -1$). An exact statement will be given in \cref{def:probSolNoTens,def:probSolTension}. 
While probabilistic solutions of the Stefan problem are well understood in one space dimension \cite{DNS,CRS} and for  radially symmetric solids \cite{ MishaRadialTension}, less is known in the general case.  Additional challenges arise  when  incorporating surface tension %$-$otherwise called \textit{Gibbs-Thomson}$-$
effects \cite{Almgren, Popinet,  MishaRadialTension}. The so-called \textit{Gibbs-Thomson law} states that the temperature at the interface is below (resp. above) the usual melting point where the solid is locally convex (resp. concave).   

 
   % \begin{equation*}
   %     \int_{\Gamma_{0-}}\psi -  \int_{\Gamma_t  } \psi 
   % = \E^{\mu^1}[  \psi(X_{\tau^1}^1)\mathds{1}_{\{ \tau^1 \le t\}}] - \E^{\mu^2}[  \psi(X_{\tau^2}^2)\mathds{1}_{\{ \tau^2 \le t\}}], 
   % \end{equation*}  whatever test function $\psi$. 


The goal of this work is to characterize \text{probabilistic} solutions of general  Stefan problems   where the full theory is still to be  established.  Precisely, we  represent $\Gamma = (\Gamma_t)_{t\in [0,T]}$,  the evolving region occupied by the solid, using %and advocate 
the celebrated \textit{level-set method} \cite{OsherSethian}. % to perform such a task. 
Specifically, the evolving solid corresponds to the zero sublevel sets of some  auxiliary function $\Phi: [0,T] \times \R^d \to \R$, focusing on $d\in \{2,3\}$ in our  numerical experiments. 
The level-set method is a popular approach to describing the evolution of moving  interfaces in arbitrary dimensions. %In the applications, the interface may represent the front of a wildfire 
Moreover, it  requires no assumptions on the geometry of the unknown  region and  can easily handle changes in topological properties. % over time.
For instance, level sets can capture the separation of a connected set into several components and vice versa. % as we shall see in \cref{sec:Dumbbell} describing the melting of a dumbbell-shaped solid. %deal with changes in topological properties such as connectedness. %represent disconnected regions and more general topological changes.    
As we shall see in the numerical examples (\cref{sec:Dumbbell}), this flexibility is necessary for general Stefan problems.  We refer the reader to the excellent books of \citet{OsherFedkiw} and \citet{Sethian} for a comprehensive description of level-set methods.  

To the best of our knowledge, the use of the level-set method for the Stefan problem was first  proposed by \citet{OsherStefan}.  Their algorithm alternately  approximates the moving front through level-set functions and the temperature   in each phase using a finite difference scheme for the corresponding heat equation. The method is capable of  accurately reproducing known solutions to the Stefan problem as well as generating realistic dendritic growth for various solids.  See also \cite{Gibou} focusing on dendritic crystallization and \cite[Section 23]{OsherFedkiw} presenting applications to general heat flows. 
Here, the level-set function is parameterized by a time-space feedforward neural network $\Phi:[0,T]\times \R^d \times \Theta \to \R$ where $\Theta$ is a finite-dimensional  parameter set.  The parameters are trained using stochastic gradient descent by converting the growth condition of probabilistic solutions %(see \cref{def:probSolNoTens}) 
into a loss function.  
The computation of the latter involves the simulation of reflected Brownian particles in both the liquid and solid phases. The proposed method has the advantage that the normal vector to the interface$-$which is essential in level-set methods$-$can be effortlessly computed through automatic differentiation of the deep level-set function. 

The training of neural network parameters is made available via a relaxation of the loss function entailing stopped particles. Indeed, the hitting time of sharp interfaces will result in vanishing gradient issues and prevent the deep level-set function to train.  The same procedure is applied in \cite{ReppenSonerTissotFB,ReppenSonerTissotDF,SonerTissot} in the context of optimal stopping where the neural network approximates the free boundary directly. The relaxation consists of  introducing a \textit{mushy region} separating the solid and liquid as in phase-field models  \cite{BSS,B-mushy,SonerMS}. 
%Moreover,  our approach is meshfree so it can be easily generalized to higher dimensions. %In particular, the front $\partial \Gamma$ need  not be tracked explicitly. 
We also stress that the  temperature need not be approximated during training. Due to the probabilistic nature of the algorithm, the temperature can later be estimated from the density of surviving particles. Moreover, our algorithm can handle surface tension effects, as we shall see in \cref{sec:MethodTension}. We refer the interested reader to \cite{Popinet} surveying computational methods for differential equations in fluid mechanics with surface tension.

Solving free boundary problems with   the level-set method and deep learning appears to be new. Our work shares some similarities \cite{Angelo}  solving controlled front propagation flows with the level-set method where the velocity$-$the control$-$is approximated by neural networks. Yet,  the level-set function  is not parameterized directly. 
The present approach is motivated by recent 
advances of deep learning to solve complex and/or high-dimensional problems in partial differential equations \cite{HanJentzenE,DGM,WangPerdikaris,PhamPDE}, optimal stopping \cite{Becker1,Becker2,ReppenSonerTissotFB,ReppenSonerTissotDF}, and general stochastic control problems \cite{HanE,PhamNum,ReppenSonerTissotDF}. To describe physical phenomena, %the introduction of  
\textit{physics-informed} neural networks \cite{PerdikarisPI,WangPerdikaris} successfully combines observed data with known physical laws to learn the solution to a variety of problems in physics. %Stokes equation  
%opened the doors to many applications. 
governing phenomena such as fluid dynamics, heat transfer, and flow mechanics. 
The neural parameterization of level-set functions has already shown promising results in computer vision. Among others, a neural network is trained to approximate the signed distance function associated with three-dimensional objects \citet{DeepSDF} or their "occupancy probability" \citet{OccupancyNN}.  

We believe that the proposed deep level-set method can be applied to problems in different contexts. %will open the doors to other applications. % where the geometry of the free boundary is unknown. %Examples include free boundary problems arising from Hele-Shaw and Stokes flow \cite{Howison}, the pricing of  general American financial derivatives \cite{ReppenSonerTissotFB}, or   portfolio choice problems with transaction costs \cite{MKRS}. 
This includes  free boundary problems in physics, such as  Hele-Shaw and Stokes flow \cite{Howison}.  In mathematical finance, the method can also be used to generalize the "neural optimal stopping boundary method" \cite{ReppenSonerTissotFB} parameterizing the exercise boundary of American options with known geometric structure. Also, optimal portfolio problems with transaction costs \cite{MKRS} could benefit from our method if the so-called no-trade zone is represented by a deep level-set function.  % In mathematical finance, the method can be adapted to describe the stopping region of American options and  thus extending  when the geometric structure of the exercise boundary is boundary.  Another application would be to represent 

\textbf{Structure of the paper.} We introduce the Stefan problem and probability solutions  in \cref{sec:Problem}. The deep level-set method is described in \cref{sec:Method} and extended in \cref{sec:MethodTension} for the Stefan problem with  surface tension.     \cref{sec:Numerics} is devoted to the numerical results in the radially symmetric case (\cref{sec:RadialNumerics}) and for  general shapes of the solid (\cref{sec:GeneralNumerics}).  \cref{sec:conclusion} concludes the study and \cref{app:Proofs} contains the proofs of the main results. 

\textbf{Notations.}  Given a Lebesgue measurable set $A\subset \R^d$, $d\ge 1$, and measurable function $\psi:\R^d\to \R$, we employ the short notation $\int_A \psi= \int_A \psi(x)dx$ and $\int_{\partial A} \psi =  \int_{\partial A}\psi(x)d\calH^{d-1}(x)$ where $\calH^{s}$ is the $s-$dimensional Hausdorff measure. We also write $|A| = \calH^d(A)$ for the Lebesgue measure of $A$. 

==> Method.tex <==
\section{Deep Level-Set Method} \label{sec:Method}
% The level-set method is a popular approach to describing the evolution of moving  interfaces and require little assumptions on the topology of the unknown region. For instance, level sets can easily represent  disconnected regions. As we shall see in the numerical examples, this flexibility is necessary for the Stefan problem.  We refer the reader to the excellent book \cite{OsherFedkiw} for a comprehensive description of level-set methods.  
Let  $\Gamma = (\Gamma_t)_{t\in [0,T]}$ be the time-varying region occupied by the solid and consider a \textit{level-set function} $\Phi: [0,T]\times \Omega \to \R$ such that 
$$  \Gamma_t = \{x \in \Omega \ : \ \Phi(t,x) \le 0\}. $$ The free boundary $\partial \Gamma_t$ therefore corresponds to the zero isocontour $\{\Phi(t,\cdot) = 0\}$. 
 We also assume that the initial region $\Gamma_{0-}$ is embedded as the zero sublevel-set of some function $\Phi_0: \Omega \to \R$.  
Whenever $\Phi \in \calC^{1,2}([0,T]\times \Omega;\R)$ and $\nabla \Phi\neq 0$,  the normal speed, outer normal vector, and mean curvature  of $\Gamma$  read\footnote{The factor $\frac{1}{d-1}$ in the mean curvature  ensures that $\kappa_{\partial B}(x) = \frac{1}{|x|}$   for any ball  $B \subset \R^d$. } 
$$V = - \frac{\partial_t \Phi}{|\nabla \Phi|}, \quad \nu = \frac{\nabla \Phi}{|\nabla \Phi|}, \quad \kappa_{\partial \Gamma} = \frac{\text{div}(\nu)}{d-1}. $$
In particular,  the Stefan condition \eqref{eq:2SPStefan} can be rewritten as 
 \begin{equation*}
     \partial_t \Phi = \frac{\alpha_1}{2L}  \nabla \Phi \cdot \nabla u^1 - \frac{\alpha_2}{2L} \nabla \Phi \cdot \nabla u^2. 
 \end{equation*}
%the outer normal vector field to $\Gamma$  can be expressed as $\nu = \frac{\nabla \Phi}{|\nabla \Phi|}$ and the velocity  as $V = - \frac{\partial_t \Phi}{|\nabla \Phi|}$. %For instance, the gradient $\nabla \Phi$ (when it exists) is a unit vector, and therefore coincide with the  outer  normal to the interface.   
Note that level-set functions always exist, e.g. consider  the \textit{signed distance function} $$\bar{\Phi}(t,x) := (-1)^{\mathds{1}_{\Gamma_{t}}} d(x,\partial \Gamma_{t}). $$ %Whenever possible,  the level-set function describing $\Gamma_{0-}$ is given by \textit{signed distance} to the phase boundary from the  
The signed distance function possesses many suitable properties; see   \cite[Section I.2]{OsherFedkiw}. In particular, $\bar{\Phi}$ solves the Eikonal equation $|\nabla \bar{\Phi}| =1$ when  $ \bar{\Phi}$ is differentiable. Hence the gradient of signed distance function coincides with the outer normal vector $\nu$.    
 When  $\bar{\Phi} \in \calC^{1,2}([0,T]\times \Omega;\R)$, this also implies that  $V = -\partial_t \bar{\Phi}$ and  $\kappa_{\partial \Gamma} = \frac{\Delta \bar{\Phi}}{d-1}$.  

To approximate a general level-set function $\Phi$,  we parameterize the difference   $\Phi(t,\cdot) - \Phi_0$  with a neural network $  G:[0,T]\times \Omega \times \Theta \to \R$, for some   parameter set $\Theta\subset \R^p$, $p\in \N$. This leads to  the \textit{deep level-set function}  
\begin{equation}\label{eq:deepLevelSet}
    \Phi(t,x;\theta) := \Phi_0(x) + G(t,x;\theta) , \quad t\in [0,T], 
\end{equation} 
with the associated  regions $ \Gamma^{1,\theta} = \{\Phi(\cdot \ ;\theta) > 0\}$ and  $\Gamma^{\theta} =\Gamma^{2,\theta} = \{\Phi(\cdot \ ;\theta) \le  0\}$. The main reason behind parameterizing the difference is that the initial condition holds automatically. This is also convenient to capture occasional jumps in the solid region at $t=0$ when the initial data $(u_0^1,u_0^2)$ exhibit discontinuities; see \cref{sec:jumpExample}. 
 
%Indeed, $G(t,\cdot)$ can be initialized  anywhere close to $0$ so that the liquid region does not change dramatically after the initial time. The network will then  gradually adjust  to capture melting rate of the solid region.

\begin{example}\label{ex:radial}
(Radial case) Let $\Omega = B_R := \{|x|\le R\}$ and $\Gamma_{0-} =  B_{r_0}$ for some $r_0 \in (0,R)$. We can therefore initialize the level-set function with the signed distance  $\Phi_0(x) = |x| - r_0$. If the initial temperature inside the solid and liquid is radially symmetric, then $\Gamma_t =  B_{r(t)}$ for some càdlàg function $r:[0,T] \to [0,R]$. We can therefore set $\Phi(t,x) = |x| - r(t)$, as illustrated in \cref{fig:levelSetViz}. This implies that
$\Phi(t,x) - \Phi_0(x) = r_0 - r(t)$ for all $x \in \Omega.$ 
Hence the  neural network, although unaware of the radial symmetry,  "simply" needs to learn a function of time.  
\end{example}

\begin{figure}[t]
    \centering
    \caption{Time evolution of the level-set function  in the radial case  and projected solid region (bottom horizontal plane).  }
    \includegraphics[height = 1.9in,width = 6in]{Figures/Level-set Function.png}
\label{fig:levelSetViz}
\end{figure}

\subsection{Loss Function and Training}
Let us explain how the parameters in $\Gamma^{\theta}$ can be trained so as to find a probabilistic solution. 
Quite naturally, we first transform the growth condition \eqref{eq:probaCond2} into a loss function. 
If $\Psi \subseteq \calC_c^{\infty}(\Omega)$ is a finite collection of  test functions, we therefore  aim to 
\begin{equation}\label{eq:minimization}
    \text{minimize }\; \calL(\theta) = \sum_{\psi\in \Psi} \calL(\theta, \psi) \; \text{ over } \; \theta \in \Theta, \quad \text{where}
\end{equation}
\begin{align}\label{eq:loss}
    \calL(\theta,\psi) =  \left \lVert  \int_{\Gamma_{0-}} \psi - \int_{\Gamma^{\theta}_{\cdot}} \psi   -  \frac{1}{L} \left[ \eta\  \mathbb{E}[\psi(X^1_{\tau^{1,\theta}})1_{\{\tau^{1,\theta} \  \le \ \cdot\}}] -  \mathbb{E}[\psi(X^2_{\tau^{2,\theta}})1_{\{\tau^{2,\theta} \  \le \ \cdot\}}] \right] \right \rVert_{L^2([0,T])}^2. 
\end{align} 
  We therefore expect that $\Gamma^{\theta}$ induces a probabilistic solution if $\calL(\theta)=0 $ and  $\Psi$ grows to (a dense subset of) $\calC_c^{\infty}(\Omega)$. To compute the loss function in \eqref{eq:minimization},  we simulate reflected Brownian particles $X^j = (X_{t_n}^j)_{t_n \in \Pi^N}$, $j=1,\ldots,J$, on a regular time grid $\{t_n = n\Delta t \ : \ n=0,\ldots, N \}$, $\Delta t = \frac{T}{N}$,  and batch size $B\in \N$. This gives the empirical loss 
\begin{align}
    \calL(\theta) &= \sum_{\psi\in \Psi} \sum_{n=1}^N \ell_{n}(\theta,\psi)^2,  \label{eq:totalLoss}\\[0.4em]
    {\scriptsize \ell_n(\theta,\psi)} &=  \scriptsize \int_{ \Gamma_{0-}} \psi   - \int_{\Gamma^{\theta}_{t_n}} \psi   - \ \frac{1}{JL}\sum_{j=1}^J\left[\eta \ \psi(X^{1,j}_{\tau^{1,\theta,j}})\mathds{1}_{\{\tau^{1,\theta,j}  \le t_n\}} - \ \psi(X^{2,j}_{\tau^{2,\theta,j}})\mathds{1}_{\{\tau^{2,\theta,j}  \le t_n\}}\right] . \label{eq:partialLoss}
\end{align}
%To minimize stochastic gradient descen
We then aim to train  the deep level-set function with stochastic gradient techniques. That is, the parameters are updated according to 
\begin{equation}\label{eq:SGD}
    \theta_{m+1} = \theta_{m} - \zeta_m \nabla_\theta \calL(\theta_m), \quad  m = 1, \ldots, M,
\end{equation}
for some $M\in \N$. However, the map $\theta \mapsto \tau^{\theta}$ is piecewise constant, where $\tau^{\theta}$ denotes a  stopping time on the right-hand side of \eqref{eq:partialLoss}. For concreteness, let us suppose that $\tau^{\theta}$ is the exit time of a liquid particles from the liquid region. In terms of the parameterized level-set function, this reads
$$\tau^{\theta} = \inf\{t_n, n\le N \ : \ \Phi(t_n,X_{t_n}^1;\theta) < 0\}. $$
Unless a trajectory $(X_{t_n}(\omega))_{n=0}^N$ is exactly on the solid-liquid interface at the stopping time $\tau^{\theta}(\omega)$, i.e. $\Phi(\tau^{\theta}(\omega),X_{\tau^{\theta}}^1(\omega);\theta)=0$,  the value of $\tau^{\theta}(\omega)$ will remain the same after an infinitesimal change in the parameter vector $\theta$. 
Hence, stochastic gradient descent would not converge as the gradient $\nabla_{\theta} \tau^{\theta}$ vanishes almost everywhere. To circumvent this issue, the stopping times need to be relaxed as explained in the next section. 

Regarding the test functions, we choose  the Gaussian kernels\footnote{If $\beta_k$ is large enough, then, at least numerically,  $\psi_k$ is  compactly supported in $\Omega$. }   
 $$\Psi = \left\{\psi_k(x) = e^{-\beta_k |x-z_k |^2} \ : \  \beta_k >0, \ z_k\in \Omega, \  k=1,\ldots, K \right\}, \quad K\in \N.$$
The centers $z_k$ and width $\beta_k$  are randomized  at each training iteration to cover the whole domain and capture various scales. 
 \subsection{Relaxed Stopping Times}

 We adapt the relaxation procedure proposed in \cite{ReppenSonerTissotFB} in the context of optimal stopping problems. In short, it consists of replacing the sharp boundary $\partial \Gamma_t$ by a \textit{mushy} (or \textit{fuzzy}) \textit{region} where stopping may or may not take place.   
 First, we transform the neural network $\Phi(t,\cdot\ ;\theta)$ to locally approximate the signed distance to the interface $\partial \Gamma_t$. This is achieved by normalization, namely  by setting  $\bar{\Phi}(t,\cdot \ ; \theta) := \frac{\Phi(t,\cdot\ ;\theta)}{|\nabla_x \Phi(t,\cdot\ ;\theta)|}$.\footnote{Indeed, write $\phi = \Phi(t,\cdot\ ;\theta)$  and  fix $x \notin  \partial \Gamma_t$, i.e. $\phi(x) \ne 0$. If $\nu$ is the outer normal vector of $\partial \Gamma_t$,  the signed distance $\delta \in \R$ of $x$ to $A$ can be characterized as the smallest solution (in absolute value) to  $\phi(x - \delta \nu) = 0$. A Taylor approximation gives $0 = \phi(x - \delta \nu) \approx \phi(x) - \delta \ \nu \cdot \nabla \phi(x)$ so  $\delta \approx  \frac{\phi(x)}{|\nabla \phi(x)|}$ as desired. Note that this approximation is only accurate close to the interface, %(i.e. for small $\delta$), 
 which is precisely where the signed distance plays a role  in the algorithm. } We note that the spatial gradient of $\Phi(\cdot; \theta)$ can be exactly and effortlessly computed using automatic differentiation.  

 Next, the signed distances are converted into  stopping intensities. Without loss of generality, we describe the procedure for liquid particles which are stopped when entering the solid. For solid particles, see \cref{rem:solidParticles}. Given $\varepsilon > 0$, define the phase indicator variables 
  $$q^{\theta,\varepsilon}_n = (\chi^{\varepsilon} \circ \bar{\Phi})(t_n,X_{t_n}^1;\theta),  \quad n = 0,\ldots,N, $$
 % $$q^{\theta,\varepsilon}(t,x) = (\chi^{\varepsilon} \circ \delta)(t,x;\theta),  \quad (t,x) \in [0,T] \times \Omega, $$
% $$q^{\theta,\varepsilon}(t_m = h^{\varepsilon}  (\delta(t_m,X_{t_m};\theta)), \quad h^{\varepsilon}(\delta) = \frac{(1 - \delta/\varepsilon)^+}{2} \wedge 1. $$
with the \textit{relaxed phase function} $\chi^{\varepsilon}(\phi) = \frac{(1 - \phi/\varepsilon)^+}{2} \wedge 1$; see   \cref{fig:hFunction} for an illustration. The phase indicator variable is equal to $1$ in the "$\varepsilon-$interior" of the solid region (where $\bar{\Phi}(t,x;\theta) \le \varepsilon$) and is $0$ when $\bar{\Phi}(t,x;\theta) \ge \varepsilon$. 
The parameter $\varepsilon>0$ specifies the width of the \textit{mushy region} $$\partial \Gamma_t^{\theta,\varepsilon} = \{x \in \Omega \ : \ |\bar{\Phi}(t,x;\theta)| < \varepsilon \},$$ in which a liquid particle enters the solid region with  "probability" $q^{\theta,\varepsilon}_m \in (0,1)$. 
%In the "$\varepsilon-$interior" of the solid region, where $\chi^{\varepsilon}=1$,  the liquid particles are stopped with probability one.
Inside  $\partial \Gamma_t^{\theta,\varepsilon}$, the phase indicator variable decreases linearly with the signed distance to the interface. % and becomes zero in the "$\varepsilon-$interior" of the liquid region (where $\chi^{\varepsilon}=0$).  

For Brownian particles, a natural choice for $\varepsilon$  is $\varepsilon = \sqrt{d \ \Delta t}$, being roughly the expected euclidean distance travelled by a $d$-dimensional standard Brownian motion over one time subinterval $[t,t+\Delta t]$. For Brownian particles with diffusivity $\alpha >0$, we set instead $\varepsilon  = \sqrt{\alpha d \Delta  t}$.
When the liquid and solid particles have different diffusivities, we therefore consider distinct mushy regions.  
Finally, the stopped values in \eqref{eq:partialLoss} are  replaced by
$$\psi(X_{\tau^{1,\theta}}^1)1_{\{\tau^{1,\theta} \  \le \ t_n\}} \approx  \sum_{l=1}^n Q^{\theta,\varepsilon}_l \ \psi(X_{t_l}^1),$$
with the random stopping probabilities recursively given by
$$\quad Q_{n}^{\theta, \varepsilon} = q^{\theta,\varepsilon}_n\underbrace{\Big(1- \sum_{l<n} \ Q_{l}^{\theta, \varepsilon}  \Big)}_{\text{same phase until $t_n$}}, \quad n = 0,\ldots, N. $$%}_{\text{change phase at  $t_m$}}  

  Similarly, the integrals in \eqref{eq:partialLoss} are computed  as  
  \begin{equation}\label{eq:intMC}
      \int_{\Gamma_{t_n}^{\theta}} \psi \ \approx \  
  \frac{|\Omega|}{J}\sum\limits_{j=1}^{J} q_{n,0,j}^{\theta, \varepsilon}\ \psi(U^j), \quad   \  q_{n,0,j}^{\theta, \varepsilon} = (\chi^{\varepsilon} \circ \bar{\Phi})(t_n,U^j;\theta), \quad  U^j \overset{\text{i.i.d.}}{\sim} \ \text{Unif}(\Omega). 
  \end{equation}
 Notice that the terms $\int_{ \Gamma_{0-}} \psi_k $  do not depend on $\theta$ so they can  be computed only once, e.g. in an offline phase. 
Because of the above relaxation, the gradient of $\calL(\theta)$ does not vanish anymore. We can therefore apply stochastic gradient descent to minimize the loss function and in turn approximate the solid region $\Gamma$.  
\begin{figure}[t]
     \centering
     \caption{Illustration of the relaxed phase function $\chi^{\varepsilon}(\phi) = \frac{(1 - \phi/\varepsilon)^+}{2} \wedge 1$.}
     \includegraphics[height = 1.9in,width = 2.5in]{Figures/PhaseIndicator.pdf}
     \label{fig:hFunction}
 \end{figure}
 
% \subsection{Jump penalty}
% Set
% $\bar{\calL}(\theta) = \calL(\theta) + \zeta \calP(\theta)$, where $\zeta>0$ is a tuning parameter and 
% \begin{equation}\label{eq:symdiff}
%     \calP(\theta) = \sum_{n=1}^N \left(\frac{|\Gamma^{\theta}_{t_n} \triangle \Gamma^{\theta}_{t_{n-1}}|}{\Delta t}\right)^{p} \Delta t \ \overset{?}{\approx} \int_0^T \int_{\partial \Gamma_t} V_t^4 d\calH^{d-1} dt ,
% \end{equation}
% for some $p>0$. 

\begin{remark}\label{rem:solidParticles}
For solid particles,  the phase indicator variables are defined analogously by $$q^{\theta,\varepsilon}_n = 1 - (\chi^{\varepsilon} \circ \bar{\Phi})(t_n,X_{t_n}^2;\theta).$$ We can thereafter follow the  steps above to approximate the stopped values $\psi(X_{\tau^{2,\theta}}^2)1_{\{\tau^{2, \theta} \  \le \ t_n\}}$.
\end{remark}

\subsection{Jump penalty}\label{sec:jumpPenalty}
So far, there is no control on the change in volume of the solid region. Although jumps can be observed \cite{DNS} we may find a solution which satisfies the growth condition but exhibits non-physical jumps, i.e. of non-physically large size. To deal with this issue, we consider the more general loss function 
$\underline{\calL}(\theta) = \calL(\theta) + \lambda \calP(\theta)$, with penalty term
% \begin{equation}\label{eq:symdiff}
%     \calP(\theta) =  (\Delta t)^{-\beta}\left(\max\limits_{n=1,\ldots,N} |\Gamma^{\theta_m}_{t_n} \triangle \Gamma^{\theta_m}_{t_{n-1}}| - C \right)^+  , \quad C >0, \ \beta \in (0,1], %\max_{n=1,\ldots,N} \left(\frac{|\Gamma^{\theta}_{t_n} \triangle \ \Gamma^{\theta}_{t_{n-1}}|}{\sqrt{\Delta t}} - C \right)^+
% \end{equation}
% OR better:
% \begin{equation}\label{eq:symdiff}
%     \calP(\theta) =  \left( \frac{\max\limits_{n=1,\ldots,N} |\Gamma^{\theta_m}_{t_n} \triangle \Gamma^{\theta_m}_{t_{n-1}}|}{\Delta t^{\ \beta}} - C \right)^+  , \quad C >0, \ \beta \in (0,1], 
% \end{equation}
% \begin{equation}\label{eq:symdiff}
%     \calP(\theta) =  \left( \max\limits_{n=1,\ldots,N} |\Gamma^{\theta}_{t_n} \triangle \Gamma^{\theta}_{t_{n-1}}| - C \right)^+  , \quad C >0, 
% \end{equation}

\begin{equation}\label{eq:penalty}
    \calP(\theta) =  \rho\left( \max\limits_{n=1,\ldots,N} |\Gamma^{\theta}_{t_n} \triangle \Gamma^{\theta}_{t_{n-1}}| - C \right)  , \quad C >0, \quad \rho(\Delta) = \Delta^+ - 0.01\Delta^-, 
\end{equation}
where $\triangle$ is the symmetric difference operation, and $C > 0$ is a constant describing the  "allowed" displaced volume between time steps. We note that $\rho$ is the so-called \textit{Leaky ReLU} activation function, whose chosolid is justified as follows.  If the maximum change in volume exceeds the threshold $C$,  the deep level-set function is  severely penalized by the "ReLU" part of $\rho$ (namely $\Delta^+$). On the other hand, the "leaky" part of $\rho$, i.e. when $\Delta < 0$, is introduced to slightly incentivize the solid region to shrink/grow smoothly over time. % instead of abruptly. 

%where $\triangle$ denotes the symmetric difference. 
 % Indeed, it can be shown \bb{[...]} that the change in volume between consecutive time steps$-$namely $|\Gamma^{\theta}_{t_n} \triangle \ \Gamma^{\theta}_{t_{n-1}}|-$is of order at most $\calO(\Delta t)$.  
 
 The Lagrange multiplier $\lambda$ is decomposed into  the product of a fixed ratio $\lambda_0 > 0$  (typically less than one) and a dynamically updated factor $\lambda^{\text{\tiny  scale}}$  such that  $\lambda^{\text{\tiny scale}} \ \nabla_{\theta} \calP(\theta)$ %persistently 
 matches the scale of  the gradient $\nabla_{\theta}\calL(\theta)$. For this task, we employ the  "learning rate annealing algorithm"  outlined in  \citet{WangLearningRate}. It is a popular normalization technique for physics-informed neural networks when the loss function  comprises heterogeneous components.  Finally, the volume of $\Gamma^{\theta}_{t_n} \triangle \ \Gamma^{\theta}_{t_{n-1}}$ is estimated using Monte Carlo simulations as in \eqref{eq:intMC}. 

  Throughout the numerical experiments, we set the jump  threshold to $C = \frac{|\Omega|}{2}$. In other words, the solid region is told to grow/shrink by at most half the size of the domain per time step. This is a loose constraint, which nevertheless rules out undesirable time discontinuities as we shall see in the numerical experiments. %bringing both regularity and plenty of freedom to the parametrized level-set function. 
 At the same time, we shall see in \cref{sec:jumpExample} that the regularized algorithm is still capable of producing 
 \textit{physical jumps}, whose definition is now recalled. We also refer the interested reader to \cite{MishaRadialTension}. 
Let us focus on the radial case and consider the annuli
\begin{equation}\label{eq:annuli}
    A_{r,\Delta } :=B_{r}  \ \triangle \  B_{r+\Delta  }, \quad r\ge 0, \ \Delta \in \R. % \Delta \in [-r,\infty), \quad r .
\end{equation}
If $\Delta < -r$, then  $A_{r,\Delta } = \varnothing$.  
Then a radial solution $(\Gamma_t)_{t\in [0,T]} = (B_{r(t)})_{t\in [0,T]}$ to the Stefan problem is \textit{physical} if for all $t\in [0,T]$, the jump $\Delta r (t) = r(t) - r(t-)$ (if any) satisfies 
\begin{align}\label{eq:physicalJump}
\Delta r(t) &= \begin{cases} 
\inf\left\{\Delta > 0 \ : \  |A_{r(t-),\Delta }| > -\frac{1}{L}\int_{A_{r(t-),\Delta  }}   u^1(t-,x)\right\}, & \text{if } $\Delta r(t) >0$, 
 \\[2em]
  \sup\left\{\Delta < 0 \ : \ |A_{r(t-),\Delta }| <  \frac{1}{L}\int_{A_{r(t-),\Delta  }} |u^2(t-,x)| \right\}, & \text{if } $\Delta r(t) < 0$. 
    \end{cases} 
\end{align}
% \begin{align}\label{eq:physicalJump}
% \Delta r(t) &= \begin{cases} 
% \inf\left\{\Delta > 0 \ : \  |A_{r(t-),\Delta }| > \frac{1}{L}\int_{A_{r(t-),\Delta  }} \left(-\frac{\gamma}{|x|} - u^1(t-,x)\right) \right\}, & \text{if } $\Delta r(t) >0$, 
%  \\[2em]
%   \sup\left\{\Delta < 0 \ : \ |A_{r(t-),\Delta }| > \frac{1}{L}\int_{A_{r(t-),\Delta  }} \left(u^2(t-,x) +\frac{\gamma}{|x|}\right) \right\}. & \text{if } $\Delta r(t) < 0$. 
%     \end{cases} 
% \end{align}

When the supremum in \eqref{eq:physicalJump} is taken over an empty set, this means that the solid region melts completely at time $t$, i.e. $r(t) = 0$. 
If $t$ is a discontinuity point of $r(\cdot)$, we gather that for physical solutions, the jump size $\Delta r(t) \ne 0$ is the smallest solution (in absolute value) of 
\begin{align}
|A_{r(t-),\Delta }|&=  -\frac{1}{L}\int_{A_{r(t-),\Delta }} u^1(t-,x) , && \Delta r(t) > 0,%\in [-r(t-),0)
 \label{eq:eqPosJump} \\[1em]
  |A_{r(t-),\Delta }| &= \frac{1}{L}\int_{A_{r(t-),\Delta  }} |u^2(t-,x)| , && \Delta r(t) < 0. \label{eq:eqNegJump} 
\end{align}
% \begin{align}
% |A_{r(t-),\Delta }|&=  \frac{1}{L}\int_{A_{r(t-),\Delta }} \left(-\frac{\gamma}{|x|} - u^1(t-,x)\right) , && \Delta r(t) > 0,%\in [-r(t-),0)
%  \label{eq:eqPosJump} \\[1em]
%   |A_{r(t-),\Delta }| &= \frac{1}{L}\int_{A_{r(t-),\Delta  }} \left(u^2(t-,x) +\frac{\gamma}{|x|}\right), && \Delta r(t) < 0. \label{eq:eqNegJump} 
% \end{align}
  The left-hand side in \eqref{eq:eqPosJump}, \eqref{eq:eqNegJump} is the volume  absorbed by the solid region $\Gamma$ at time $t$. 
The right-hand side of \eqref{eq:eqPosJump},  \eqref{eq:eqPosJump} is the  aggregate change in temperature in the liquid and solid phase, respectively. %between $u_0^2$ and  $-\frac{\gamma}{|x|}$. 
%Both equations are in fact particular cases of the growth condition \eqref{eq:probaCond2}, obtained by choosing the test function $\psi\equiv 1$ over the infinitesimally small  interval $[t-,t]$. 

\begin{remark}
In the non-radial case, it is not sufficient to consider time change in volume only. The formulation of an appropriate physical condition is in fact subject of ongoing research.
\end{remark}

 \subsection{Algorithm} 

The deep level-set method is summarized in \cref{alg:DLSM1}. The learning rate process $(\zeta_{m})_{m=1}^M$ is computed using the Adam optimizer \cite{Kingma}. For the Monte Carlo simulation of particles, we use antithetic sampling  to explore the domain in a symmetric fashion as well as speed up computation. Precisely, we simulate two antithetic particles  for each generated initial point $x_0^i$, namely  
\begin{align*}
    X^i &= x_0^i + \sqrt{\alpha_i} \ W_{\cdot\wedge \tau^i}^i + l_{\cdot\wedge \tau^i}^i, \quad 
    \tau^i = \inf\{t\in [0,T] \ | \ X_t^i \notin \Gamma_t^i \},\\[0.5em]
    \tilde{X}^i &= x_0^i - \sqrt{\alpha_i} \ W_{\cdot\wedge \tilde{\tau}^i}^i + \tilde{l}_{\cdot\wedge \tilde{\tau}^i}^i, \quad 
   \tilde{\tau}^i = \inf\{t\in [0,T] \ | \ \tilde{X}_t^i \notin \Gamma_t^i \}. \quad (\tilde{l}: \text{local time of $\tilde{X}^i$ at $\partial \Omega$})
\end{align*}

\begin{algorithm}[T]
\caption{(Deep Level-set method for the classical Stefan problem ) }\label{alg:DLSM1} % Training of the deep level-set function
\vspace{1mm}
\textbf{Given}: $\Phi_0=$ initial level-set  function, $J=$ batch size, $M=$ \# training iterations, $\Psi = $ set of test functions, $C=$ jump constant, $\varepsilon=$ mushy region width.\\[-0.8em] \hline
\begin{itemize}
 \setlength \itemsep{-0.1em}
 
\item[I.] \textbf{Initialize} $\theta_0 \in \Theta$
\item[II.] For $m = 0,\ldots, M-1$:
    \begin{enumerate}
    \setlength \itemsep{0.5em}

  \item \text{\textbf{Simulate} $X^{i,j} = (X_{t_n}^{i,j})_{n=0}^N$ ($i=1$: liquid, $i=2$: solid),  $\ U^j  \ \overset{\text{i.i.d.}}{\sim} \  \text{Unif}(\Omega)$, $j=1,\ldots,J$}
  
  \item \textbf{Approximate} the signed distance function of $\Gamma$ as $\bar{\Phi}(\cdot;\theta_{m}) = \frac{ \Phi(\cdot;\ \theta_{m})}{|\nabla_x \Phi(\cdot;\ \theta_{m})|}$
  
        \item For $n=0,\ldots,N$, $\psi \in \Psi$, \textbf{compute}: 
        \begin{itemize}
         \item \textbf{Phase indicator variables:} 
        \text{$q_{n,i,j}^{\theta_{m},\varepsilon} = \begin{cases}
        (\chi^{\varepsilon} \circ \bar{\Phi})(t_n,U^j;\theta_{m}) & i=0,\\[0.2em]
             (\chi^{\varepsilon} \circ \bar{\Phi})(t_n,X_{t_n}^{1,j};\theta_{m}), & i=1,\\[0.2em]
            1-  (\chi^{\varepsilon} \circ \bar{\Phi})(t_n,X_{t_n}^{2,j};\theta_{m}), & i=2.\\
        \end{cases}$}
       \item   \textbf{Symmetric Differences:} $|\Gamma^{\theta_m}_{t_n} \triangle \Gamma^{\theta_m}_{t_{n-1}}|  \approx \frac{|\Omega|}{J}\sum\limits_{j=1}^{J} |q_{n,0,j}^{\theta_m, \varepsilon} -  q_{n-1,0,j}^{\theta_m, \varepsilon}|  $\\[-0.2em] 
                 \item   \textbf{Integrals:} $\int_{\Gamma^{\theta_m}_{t_n}} \psi \ \approx \  \frac{|\Omega|}{J}\sum\limits_{j=1}^{J} q_{n,0,j}^{\theta_m, \varepsilon}\ \psi(U^j)$\\[-0.5em]
            \item \textbf{Stopped values: } \text{$\psi(X^{i,j}_{\tau^{\theta_l}})\mathds{1}_{\{\tau^{\theta_m}   \le t_n\}} \approx \sum\limits_{l=1}^n Q_{l,i,j}^{\theta_l,\varepsilon}\psi(X_{t_l}^{i,j})$, $\; \  Q_{n,i,j}^{\theta_m,\varepsilon} = q_{n,i,j}^{\theta_{m},\varepsilon} ( 1 - \sum\limits_{l<n} Q_{l,i,j}^{\theta_{m},\varepsilon} ) $}\\[-0.2em]
  
        \end{itemize}
\item  \textbf{Loss}: $\calL(\theta_m) = \sum\limits_{\psi\in \Psi}\sum\limits_{n=1}^N\ell_n(\theta_m,\psi)^2$, with 
\begin{align*}
    {\scriptsize \ell_n(\theta_m,\psi)} &=   {\scriptsize \int_{ \Gamma_{0-}} \! \psi   - \int_{\Gamma^{\theta_m}_{t_n}} \! \psi   - \ \frac{1}{JL}\sum_{j=1}^J\left[\eta \ \psi(X^{1,j}_{\tau^{1,\theta_m,j}})\mathds{1}_{\{\tau^{1,\theta_m,j}  \le t_n\}} - \ \psi(X^{2,j}_{\tau^{2,\theta_m,j}})\mathds{1}_{\{\tau^{2,\theta_m,j}  \le t_n\}}\right] } %\textbf{Aggregate}
\end{align*}

\item \textbf{Jump penalty:} \text{ $\ \calP(\theta_m) =  \rho \left(\max\limits_{n=1,\ldots,N} |\Gamma^{\theta_m}_{t_n} \triangle \Gamma^{\theta_m}_{t_{n-1}}| - C \right)$} \\[0.1em]
\item \textbf{Gradient step:} $\theta_{m+1} = \theta_{m} - \zeta_m \nabla_\theta \underline{\calL}(\theta_m) $, $\; \underline{\calL}(\theta_m) = \calL(\theta_m) + \lambda_0 \ \lambda_m^{\text{\tiny scale}} \calP(\theta_m) $
   \end{enumerate}
\item[III.] \textbf{Return} $\Gamma^{\theta_I} = \{\Phi(\cdot \ ; \theta_{I}) \le 0\}$\\[-2em]
\end{itemize}
\end{algorithm}

\subsection{Adding surface tension} \label{sec:MethodTension}

\subsubsection{Growth Condition Revisited }
The numerical verification of the growth condition given in \cref{def:probSolTension} is not straightforward because of the additional terms $\calK_t^1, \calK_t^2$. 
It turns out that  an  alternative formulation, which we now outline, greatly simplifies the implementation. In what follows, we assume  that $d\ge 2$. % as there is no surface tension effect if $d=1$. 
For $\delta > 0$, define the one-sided mushy regions,
$$\partial \Gamma_t^{\delta, i}  = \{x\in \Gamma_t^i \ : \ d(x,\partial \Gamma_t)\le \delta \}, \quad i=1,2. $$ 

Let $(T_l^{\delta,i})_{l\ge 1}$ be the arrival times of  a time-space Poisson point process with intensity
\begin{equation}\label{eq:PoissonIntense}
     \lambda^i(t,y) = \frac{\gamma}{\delta} |\kappa_{\partial\Gamma_t}(\hat{y})|^{2-d} \frac{\mathds{1}_{\partial \Gamma_t^{\delta,i}}(y)}{|\partial \Gamma_t^{\delta,i}|},\quad \hat{y} = \text{proj}_{\partial \Gamma_t}(y), \quad d\ge 2. 
\end{equation}
 For each $l\ge 1$ and $i=1,2$, we simulate a Brownian particle $Y^{l,i} = (Y^{l,i}_s)_{s\in[T_l^{\delta,i},T]}$ where, according to \eqref{eq:PoissonIntense}, the initial position of $Y^{l,i}$ is uniformly distributed in $\partial \Gamma_{T^{\delta,i}_l}^{\delta,i}$ if $d= 2$ and inversely proportional to the absolute mean curvature of $\partial \Gamma_{T^{\delta,i}_l}$ otherwise.  
Moreover,  we define the exit times $\tau_l^{\delta,i} = \inf\{s \ge T^{\delta,i}_l \ : \ Y^{l,i}_s \notin \Gamma_s^i \}$. 

In the three-dimensional, radially symmetric case (namely $\Gamma_t = B_{r(t)} \subseteq \R^3$),  the Poisson intensities simply read
\begin{equation}\label{eq:PoissonIntenseRad}
     {\lambda^i(t,\cdot) = \frac{\gamma}{\delta}} r(t) \frac{\mathds{1}_{A_{r(t),\Delta_i}}}{|A_{r(t),\Delta_i}|}, \quad   \Delta_i = (-1)^i \delta,
\end{equation}
with the annuli $A_{r,\Delta}$ defined in \eqref{eq:annuli}. We therefore gather that the expected number of simulated particles is directly  proportional to the radius of the spherical solid region. 

% \begin{figure}[H]
%      \centering
%      \caption{Creation of new particles in the solid and liquid mushy regions (radial case) \bb{(improve, e.g. non radial example) or remove)}. }
%      \includegraphics[height = 2.0in,width = 2.4in]{Figures/Boundary Particles t = 0.0.pdf}
%      \label{fig:bdryparticles}
%  \end{figure}

\begin{proposition}\label{prop:growthCondTensionPoisson}
Consider the radially symmetric Stefan problem with  surface tension. Moreover, assume that $\alpha_1 = \alpha_2$ and let  $N_t^{\delta,i} := \sum_{l=1}^{\infty} \mathds{1}_{\{T^{\delta,i}_l \le t\}}$ be the counting process associated to $(T^{\delta,i}_l)$, $i=1,2$.  Then for all $ \psi \in \mathcal{C}_c^{\infty}(\Omega)$, 
\begin{align}
      \int_{\Gamma_{0-}}\psi -  \int_{\Gamma_t  } \psi
   &=  \frac{1}{L} \left[ \eta \E^{\mu^1}[ \psi(X_{\tau^1}^1)\mathds{1}_{\{ \tau^1 \le t\}}] - \E^{\mu^2}[  \psi(X_{\tau^2}^2)\mathds{1}_{\{ \tau^2 \le t\}}] + \calK_{t}   \right],\label{eq:probacondTension2}  \\[1em]  
  \calK_{t} &= \eta \calK_t^1 - \calK_t^2, \\[1em]
 \calK_t^i &= \lim_{\delta \downarrow 0} \  \E\left[\sum_{l = 1}^{N_t^{\delta,i} } \left( \psi(Y_{\tau_l^{\delta,i}}^{l,i}) \mathds{1}_{\{\tau^{\delta, i}_l \le t\}} \ {- \  \psi(Y_{T^{\delta,i}_l}^{l,i})}   \right)\right] \label{eq:curvatureTerm}
\end{align}
% \begin{align}
%       \int_{\Gamma_{0-}}\psi -  \int_{\Gamma_t  } \psi
%    &=  \frac{1}{L} \left[ \eta \left(\E^{\mu^1}[ \psi(X_{\tau^1}^1)\mathds{1}_{\{ \tau^1 \le t\}}] +   \calK_t^1 \right) - \E^{\mu^2}[  \psi(X_{\tau^2}^2)\mathds{1}_{\{ \tau^2 \le t\}}] - \calK_t^2   \right],\label{eq:probacondTension2} 
%  + \calK_{t}
%  \end{align}
\end{proposition}

\begin{proof}
See \cref{app:growthCondTensionPoisson}. 
\end{proof}

\begin{remark}
    When the diffusivities of the solid and liquid phase are different ($\alpha_1 \ne \alpha_2$), the right hand-side of the growth condition \eqref{eq:probacondTension2} entails an additional term, namely 
$$\tilde{\calK}_t  =  - \gamma\frac{\alpha_2-\alpha_1}{2} \int_0^t\int_{\partial \Gamma_s} \kappa_{\partial \Gamma_s} \  \partial_{\nu} \psi.$$ 

%\approx \frac{\alpha_2-\alpha_1}{4\delta} \int_0^t\int_{\partial \Gamma_s^{\delta}} u \  \partial_{\nu} \psi  = \frac{\alpha_2-\alpha_1}{2} \int_0^t\E[ \partial_{\nu} \psi(X_s) \mathds{1}_{\{\tau>s\}} ] $$

Recalling that $u^1=u^2 = - \gamma \kappa_{\partial \Gamma_s} $, the above term can be approximated as 
$$\tilde{\calK}_t \approx    \frac{\alpha_2}{2\delta } \int_0^t\int_{\partial \Gamma_s^{\delta,2}} u^2 \  \partial_{\nu} \psi - \frac{\alpha_1}{2\delta } \int_0^t\int_{\partial \Gamma_s^{\delta,1}} u^2 \  \partial_{\nu} \psi.$$ 
We can finally compute the integrals $\int_{\partial \Gamma_s^{\delta,i}} u^i \  \partial_{\nu} \psi$ using the stochastic representation of $u^i$ given in \eqref{eq:intu^i}. Note also that $\partial_{\nu} \psi$ is easily computed as the outer normal $\nu$ is available from the deep level-set function. 
\end{remark}

\begin{remark} \label{rem:curvconjecture}
It is conjectured that the representation \eqref{eq:curvatureTerm} of the curvature terms holds in  non-radial case as well. The only difference is that the effect of boundary particles is reversed in \textit{concave} sections of the boundary. Precisely, we have in general that 
\begin{equation}
    \calK_t^i &= \lim_{\delta \downarrow 0} \  \E\left[\sum_{l = 1}^{N_t^{\delta,i} } \text{sign}(\kappa_{\partial \Gamma_{ \! T_l^{\delta,i}}}(Y_{T^{\delta,i}_l}^{l,i}))\left( \psi(Y_{\tau_l^{\delta,i}}^{l,i}) \mathds{1}_{\{\tau_l^{\delta,i} \le t\}} \ - \  \psi(Y_{T^{\delta,i}_l}^{l,i})   \right)\right].\label{eq:curvatureTerm2}
\end{equation}
\end{remark}
 We show how to approximate $\calK_t^i$ given in \eqref{eq:curvatureTerm}. First, the mushy regions can be expressed in terms of  the level-set function as follows:  $$\partial \Gamma_t^{\delta,1} \approx \left \{x\in \Omega \ : \ \frac{\Phi(t,x)}{|\nabla \Phi(t,x)|} \in (0,\delta] \right\}, \quad \partial \Gamma_t^{\delta,2} \approx \left \{x\in \Omega \ : \ \frac{\Phi(t,x)}{|\nabla \Phi(t,x)|} \in [-\delta,0] \right\}.$$ 
Without loss of generality, we focus on the term $\calK_t^1$ and drop the superscripts $^1$ throughout. 
Using the time discretization  $\{t_n = n\Delta t \ : \ n=0,\ldots, N \}$, $\Delta t = \frac{T}{N}$, $N\in \N$, we obtain for $\delta>0$ sufficiently small that   
$$\calK_{t_n} \approx \ \sum_{m=0}^{n-1} \E\left[\sum_{l =N^{\delta}_{t_{m}}{+1}}^{N^{\delta}_{t_{m+1}}}  \E\big [\psi(Y_{\tau_{l}^{\delta}}^{l}) \mathds{1}_{\{\tau_{l}^{\delta} \le t_n\}}  - \psi(Y_{t_m}^{l}) \ | \ T^{\delta}_l = t_m \big ]  \right] .  $$ 
Writing $\E_{t_m,y}[\cdot ] = \E[ \ \cdot \ | \ Y_{t_m}  = y, T^{\delta} = t_m ]$ where  $Y, T^{\delta}$ has the same law as  $Y^{l},T^{\delta}_l$ for any $l\ge 1$, we obtain from Wald's identity that 
\begin{align*}
  \calK_{t_n} &\approx \ \sum_{m=0}^{n-1} \int_{\partial \Gamma_{t_m}^{\delta}}  \E_{t_m,y}[N^{\delta}_{t_{m+1}}-N^{\delta}_{t_{m}}] \E_{t_m,y}[\psi(Y_{\tau^{\delta}}) \mathds{1}_{\{\tau^{\delta} \le t_n\}}{ - \psi(Y_{t_m})} ] dy\\
  &\approx \ \sum_{m=0}^{n-1} \int_{\partial \Gamma_{t_m}^{\delta}}  \lambda(t_m,y) \E_{t_m,y}[\psi(Y_{\tau^{\delta}}) \mathds{1}_{\{\tau^{\delta} \le t_n\}}{ - \psi(Y_{t_m})} ] dy.
\end{align*}
In light of \cref{rem:curvconjecture} and the Poisson intensity in \eqref{eq:PoissonIntense}, we finally obtain 
\begin{align}\label{eq:curvCompute}
   \calK_{t_n} \approx \frac{\gamma \Delta t }{\delta}   \sum_{m=0}^{n-1}  \E[\ \text{sign}(\kappa_{\partial\Gamma_{t_m}}(Y_{t_m})) \ |\kappa_{\partial\Gamma_{t_m}}(Y_{t_m})|^{2-d}\big ( \psi(Y_{\tau^{\delta}}) \mathds{1}_{\{\tau^{\delta} \le t_n\}}{ - \psi(Y_{t_m})} \big) \ | \  T^{\delta} = t_m  \big ], 
\end{align}
which is estimated through Monte Carlo simulations. We also note that, for simplicity, the curvature in \eqref{eq:curvCompute} is evaluated at $Y_{t_m}$ instead of its projection $\hat{Y}_{t_m}$ onto $\partial\Gamma_{t_m}$. This is an accurate approximation of the "true" curvature when the width $\delta$ of the mushy region is small.  %as in \eqref{eq:PoissonIntense}. 
location of $Y$ projected value What remains is to approximate the mean curvature, as we shall see in the next section. 
%If $d=2$, only the sign of curvature is needed in \eqref{eq:curvCompute} while if $d=3$, then the inverse of the mean curvature needs to be estimated as we shall see in the next section. 

% In the radially symmetric case, we may assume for  that the parameterized region is "locally radial", i.e. $\kappa_{\partial \Gamma_t^{\theta}}(y)  = \frac{1}{|y|}$, $y\in \partial \Gamma_t^{\delta, \theta}$.  This leads to the simplified expression
% \begin{align}\label{eq:curvComputeRadial}
%    \calK_{t_n} \approx \frac{\gamma \Delta t }{\delta}   \sum_{m=0}^{n-1}  \E[|Y_{t_m}|\big ( \psi(Y_{\tau}) \mathds{1}_{\{\tau \le t_n\}}{ - \psi(Y_{t_m})} \big) \ | \  T_{\delta} = t_m  \big ].
% \end{align}
% We stress that the neural network representing the level-set function is unaware of the radial symmetry. Employing \eqref{eq:curvCompute} or \eqref{eq:curvComputeRadial} yield comparable results, as we shall see  in 
% \cref{sec:3D2PTension}. 

% \begin{example}
%     Let $d=2$ and assume that the solid region is convex. If $\psi\equiv 1$ and $\Delta t$ is small, then 
%        $$\calK_{\Delta t}^i \approx  \E\left[\sum_{l = 1}^{N_{\Delta t}^{\delta,i} } \left(  \mathds{1}_{\{\tau^{i}_l \le t\}} \ - \ 1     \right)\right] = \frac{\gamma}{\delta} \Delta t \left[  \Pb(\tau^{i}_1 \le \Delta t) - 1\right].$$
%       If $\eta=1$, the growth condition  reads
%        \begin{align*}
%            |\Gamma_{0-}| - |\Gamma_{\Delta t}| =  \Pb( \tau^1 \le \Delta t) - \Pb( \tau^2 \le \Delta t) +  \underbrace{\frac{\gamma}{\delta} \Delta t \left[\Pb(\tau^{1}_1 \le \Delta t) - \Pb(\tau^{2}_1 \le \Delta t) \right] }_{(\star)}
%        \end{align*}
%        If $\Gamma$ is convex, then the boundary particles in the solid are more likely hit the boundary than those in the liquid (which can more easily "escape"). Hence $ \Pb(\tau^{2}_1 \le \Delta t) \ge \Pb(\tau^{1}_1 \le \Delta t)$, which implies that the surface tension term $(\star)$ is negative and \rr{slows down} the melting of the solid. \bb{But numerically $ \Pb(\tau^{2}_1 \le \Delta t) \le \Pb(\tau^{1}_1 \le \Delta t)$ (especially for later times), so it melts!}

%        Now take $\Gamma_{0-} = \{|x|_1 \le r_0\} $ and $\psi = \mathds{1}_{B_{\delta}(x_0)}$, where $\Gamma_{0-} \ni x_0 = (0,r_0)$ (a corner of the the $\ell_1$ ball). Hence $B_{\delta}(x_0) \subseteq \partial\Gamma_{0-}^{\delta,1} \cup \partial\Gamma_{0-}^{\delta,2}$.  This gives, formally\footnote{we also use that $\Pb( \tau^i \le \Delta t, X_{\tau^i}^i \in B_{\delta}(x_0)) \approx 0 $ if the initial particle $X_{0}^i$ is sampled uniformly in $\Gamma^i_{0-}$.}
%         \begin{align}
%            |\Gamma_{0-} \cap B_{\delta}(x_0)| - |\Gamma_{\Delta t} \cap B_{\delta}(x_0)| &\approx   \frac{\gamma}{\delta} \Delta t \left[\Pb(\tau^{1}_1 \le \Delta t, Y_{\tau^{1}_1}^1 \in B_{\delta}(x_0)) - \Pb( Y_{0}^1 \in B_{\delta}(x_0)) \right] \label{eq:liquid}\\
%            &- \frac{\gamma}{\delta} \Delta t \left[\Pb(\tau^{2}_1 \le \Delta t, Y_{\tau^{2}_1}^2 \in B_{\delta}(x_0)) - \Pb( Y_{0}^2 \in B_{\delta}(x_0)) \right] \label{eq:solid} \\ 
%            &\approx   \frac{\gamma}{\delta} \Delta t \left[\Pb(\tau^{1}_1 \le \Delta t, Y_{\tau^{1}_1}^1 \in B_{\delta}(x_0)) - \Pb(\tau^{2}_1 \le \Delta t, Y_{\tau^{2}_1}^2 \in B_{\delta}(x_0))  \right] \label{eq:stopped}\\
%            &+ \frac{\gamma}{\delta} \Delta t \left[\Pb( Y_{0}^2 \in B_{\delta}(x_0)) - \Pb( Y_{0}^1 \in B_{\delta}(x_0))\right]. \label{eq:created}
%        \end{align}
%        Since $Y_0^i$ is uniform in $\partial \Gamma_{0-}^{\delta,i}$, $i=1,2$ and  $|\partial \Gamma_{0-}^{\delta,1}| \approx |\partial \Gamma_{0-}^{\delta,2}|$ (when $\delta \ll r_0$), 
%        $$\Pb( Y_{0}^1 \in B_{\delta}(x_0))= \frac{|\partial \Gamma_{0-}^{\delta,1} \cap B_{\delta}(x_0)|}{|\partial \Gamma_{0-}^{\delta,1}|} >  \frac{|\partial \Gamma_{0-}^{\delta,2} \cap B_{\delta}(x_0)|}{|\partial \Gamma_{0-}^{\delta,1}|} \approx \Pb( Y_{0}^2 \in B_{\delta}(x_0)). $$
% Hence the term in \eqref{eq:created} is negative. The term \eqref{eq:stopped} is a priori negative as well since solid particles close to the corner $x_0$ are more likely to hit the boundary than liquid particles. Hence,
% $$|\Gamma_{\Delta t} \cap B_{\delta}(x_0)| \ge |\Gamma_{0-} \cap B_{\delta}(x_0)|, $$
% which means that the solid region occupies a larger area inside $B_{\delta}(x_0)$, so the corner is presumably smoothed out. \rr{or the other way round: it creates fingers??}
      % Again, the liquid term (r.h.s. of \eqref{eq:liquid}) is typically negative (particles are more likely to escape) and the solid term typically positive. 
       
%\end{example}

\subsubsection{Mean Curvature  Approximation}\label{sec:trickradial}
In this section, we present simple algorithms to locally approximate the mean curvature of a manifold $\Sigma  \subset \R^d$, $d=2,3$, of codimension $1$. Other techniques, e.g. using finite difference, are discussed in \cite{Popinet}. If $\Sigma = \{\phi = 0\}$ for some level-set function $\phi \in \calC^2(\R^d;\R)$, we recall that  the mean curvature  can be expressed as
\begin{equation}
    \kappa_{\Sigma}(x) = \frac{\text{div}\left(\nu(x)\right)}{d-1}, \quad x\in \Sigma, 
\end{equation} 
with the outer normal vector field $\nu = \frac{\nabla \phi}{|\nabla \phi|} $. If $\phi$ is parameterized by a neural network, one could apply automatic differentiation to compute $\kappa_{\Sigma}$. However, computing second order  derivatives through automatic differentiation is  costly since it entails nested gradient tapes. Indeed, the machine would need to  keep track of the first order derivatives as well. Alternative approaches have been proposed to speed up computation,  e.g. \cite{DGM} using Monte Carlo techniques.  
Here, we propose a dilation approach echoing the geometric nature of curvature and solely exploiting  the gradient of $\phi$. %, so it can be applied more generally to level-set functions in $\calC^1(\R^d;\R)$.  

As a motivation, consider a circle $\Sigma_r = \partial B_r \subseteq \R^2$  of radius $r$ whose curvature is $\kappa_{\Sigma_r} = \frac{1}{r}$. One way to approximate the curvature is to look at the ratio between  arc lengths of $\Sigma_r$   and the dilated circle $\Sigma_{r+\epsilon}$ for small $\epsilon > 0$. Indeed, writing
$\Sigma_r \supseteq \calA_{r,\epsilon_0} = \{(r\cos(t\epsilon_0),r\sin(t\epsilon_0)) \ : \ t \in [0,1]\}$ for an arc with radius $r$  and angle $\epsilon_0 \in [0,2\pi)$, note that
\begin{equation}\label{eq:curvArc}
\frac{\calH^1(\calA_{r+\epsilon,\epsilon_0})}{\calH^1(\calA_{r,\epsilon_0})} = \frac{\epsilon_0(r+\epsilon)}{\epsilon_0 r} = 1 +\epsilon \ \kappa_{\Sigma_r} \; \Longrightarrow \kappa_{\Sigma_r} = \frac{1}{\epsilon}\left(\frac{\calH^1(\calA_{r+\epsilon,\epsilon_0})}{\calH^1(\calA_{r,\epsilon_0})} -1 \right).
\end{equation}
 
We can mimic this procedure for general subsets $\Sigma  \subset \R^2$, $\text{dim}_{\calH}(\Sigma) = 1$, by locally approximating $\Sigma$ by a circle. The procedure is summarized in \cref{alg:curv2D} where $\Sigma$ is  the zero level set of some function $\phi \in \calC^1(\R^2;\R)$. An illustration is also given in \cref{fig:curvApprox2D}.  When $\epsilon_0 > 0$ is small, the arc of length  in \eqref{eq:curvArc} is  accurately replaced  by a segment tangent to $\Sigma$.     We recall that the outer normal vector field  of $\Sigma$ is readily available from  the level-set function. The tangent vector field is therefore available as well. 

\begin{algorithm}[H]
\caption{(Local approximation of  curvature, $d=2$) }\label{alg:curv2D}

\vspace{1mm}
\textbf{Given}:  $\phi\in \calC^1(\Omega; \R)$ $(\nabla \phi \ne 0)$,  $ \ \Sigma = \{\phi = 0 \} $, $ \ y \in \Sigma$, $ \ \epsilon_0>0 , \ \epsilon> 0$\\[-0.8em] \hline
\begin{itemize}
 \setlength \itemsep{-0.1em}
 
\item[I.]  Pick a direction $\mu$  in  the tangent plane at $y$, i.e. perpendicular to $\nu(y) = \frac{\nabla \phi(y)}{|\nabla \phi(y)|}$ 
\item[II.] Consider \\[-2em]
\begin{enumerate}
    \item the segment $S_y \subseteq \R^2$ with endpoints $y^{\pm}= y \pm \epsilon_0 \mu$ 
    \item the dilated segment $S^{\epsilon}_y \subseteq \R^2$ with endpoints $y^{\pm} + \epsilon \  \nu(y^{\pm} )$
\end{enumerate}

\item[III.] \textbf{Compute} the ratio $\frac{\mathcal{H}^1(S^{\epsilon}_y)}{\mathcal{H}^1(S_y)} \approx 1 + \epsilon \ \kappa_{\Sigma}(y)$

\item[IV.] \textbf{Return} the curvature $\kappa_{\Sigma}(y) \approx \frac{1}{\epsilon}\left[\frac{\mathcal{H}^1(S^{\epsilon}_y)}{\mathcal{H}^1(S_y)} - 1 \right]$\\[-1em]
\end{itemize}

\end{algorithm}

A similar procedure can be undertaken in the three-dimensional case, as explained in \cref{alg:curv3D} and displayed in \cref{fig:curvApprox3D}. In short, the segments in \cref{alg:curv2D} become quadrangles   and lengths are replaced by areas. 
In Step III. of \cref{alg:curv3D}, note that the mean curvature  appears naturally in the cross product of $(1+\epsilon \kappa_{\Sigma,1})(1+\epsilon \kappa_{\Sigma,2})$, where $(\kappa_{\Sigma,i})_{i=1}^2$ are the principal curvatures of $\Sigma$. % at the point in question. 
As the principal directions are unknown in general, the algorithm picks randomly two orthogonal vectors in the plane tangent to $\Sigma$ at some point $y\in \Sigma$. This randomization has little impact on the accuracy of the obtained as we shall see in \cref{fig:curvParabol2D} and \cref{fig:curvParabol3D}. 

\begin{algorithm}[H]
\caption{(Local approximation of mean curvature, $d=3$) }\label{alg:curv3D} 
\vspace{1mm}
\textbf{Given}: $\phi\in \calC^1(\Omega; \R)$ $(\nabla \phi \ne 0)$,  $ \ \Sigma = \{\phi = 0 \} $, $ \ y \in \Sigma$, $ \ \epsilon_0>0 , \ \epsilon> 0$\\[-0.8em] \hline
\begin{itemize}
 \setlength \itemsep{-0.1em}
 
\item[I.]  Pick two directions  $\mu_1 \perp \mu_2$ in the tangent plane at $y$, i.e. perpendicular to  $ \nu(y) := \frac{\nabla \phi(y)}{|\nabla \phi(y)|}$
\item[II.] Consider\\[-2em]
\begin{enumerate}
\item the quadrangle $Q_y$ with vertices  $y_i^{\pm} = y \pm \epsilon_0 \mu_i, \ i =1,2$ 

    \item  the quadrangle $Q^{\epsilon}_y$ with vertices $y_i^{\pm} + \epsilon \  \nu(y_i^{\pm} ),\ i =1,2$ 
\end{enumerate}


\item[III.] \textbf{Compute} the ratio $\frac{\mathcal{H}^2(Q^{\epsilon}_y)}{\mathcal{H}^2(Q_y)} \approx (1 + \epsilon \ \kappa_{\Sigma,1}(y))(1 + \epsilon \ \kappa_{\Sigma,2}(y)) \approx 1 + 2 \epsilon \ \kappa_{\Sigma}(y)$

\item[IV.] \textbf{Return} the  mean curvature $\kappa_{\Sigma}(y) \approx \frac{1}{2\epsilon}\left[\frac{\mathcal{H}^2(Q^{\epsilon}_y)}{\mathcal{H}^2(Q_y)} - 1 \right]$ \\[-1em]
\end{itemize}
\end{algorithm}

\begin{figure}[h]
\caption{Dilation technique to capture the (mean) curvature of codimension $1$ boundaries in $\R^d$,  $d=2,3$. }
\vspace{-2mm}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
     \caption{$d=2$} \includegraphics[height=1.7in,width=2.2in]{Figures/curvature2D.png}
    \label{fig:curvApprox2D}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \caption{$d=3$} \includegraphics[height=1.7in,width=2.2in]{Figures/ParaboloidBest.pdf}
    \label{fig:curvApprox3D}
\end{subfigure}
\label{fig:curvApprox}
\end{figure}

    Back to the Stefan problem, we  naturally choose $\Sigma = \partial \Gamma_t$, $t\in [0,T]$, and $\epsilon \ll \epsilon_0 \ll \delta$, where $\delta$ is the width of the fuzzy regions $\partial \Gamma_t^{\delta,1}$, $\partial \Gamma_t^{\delta,1}$. Indeed, $\epsilon \ll \epsilon_0$ is imposed to gain accuracy while $\epsilon_0 \ll \delta$ ensures that the points $y^{\pm}$ in \cref{alg:curv2D} ($y_i^{\pm}$ in  \cref{alg:curv3D})  belong also to the fuzzy region for almost every $y\in \partial \Gamma_t$. 

Let us verify \cref{alg:curv2D,alg:curv3D} respectively %produces accurate estimates of the (mean) curvature 
for parabolas $\Sigma_a := \{y  \in \R^2 \ : \ y_2 = \frac{y_1^2}{a} \}$ and paraboloids $\Sigma_{a,b} := \{y  \in \R^3 \ : \ y_3 = \frac{y_1^2}{a} + \frac{y_2^2}{b} \}$ with parameters $a,b \in \R\setminus\{0\}$. 
The (mean) curvature functions are respectively given by
\begin{equation}\label{eq:curvParabolExact}
    \kappa_{\Sigma_a}(y) 
= 
    \frac{2/a}{(1+ 4y_1^2/a^2)^{3/2}}\quad  (d=2), \qquad \kappa_{\Sigma_{a,b}}(y) = \frac{\frac{4y_1^2}{a} +  \frac{4y_2^2}{b} + a + b}{ab\left(1+ \frac{4y_1^2}{a^2} +  \frac{4y_2^2}{b^2}\right)^{3/2}} \quad  (d=3).
\end{equation}
\cref{fig:curvParabol2D} shows the approximated curvature  and relative error compared to  \eqref{eq:curvParabolExact} for a parabola $(d=2)$ with parameter $a=2$. In \cref{fig:curvParabol3D}, we repeat the exercise  for a  paraboloid with parameters $(a,b)=(1,2)$ (top panels) and a hyperbolic paraboloid with  $(a,b) =(-1,2)$ (bottom panels).   As expected, we note that the error for the hyperbolic parabola  in \cref{fig::errorParaboloid2} is only sizeable along the points with  zero mean curvature. %with %saddle points \bb{[or "3D inflection points"]}.

%In the case $d=3$, \cref{fig:curvParabol} displays the estimated mean curvature in the $(y_1,y_2)$ plane and relative error for a paraboloid with parameters $(a,b)=(1,2)$.  \cref{fig:curvHyperParabol} treats the case of  a hyperbolic paraboloid with parameters $(a =-1,b=2)$. 

% \begin{table}[H]
% \begin{center}

% \begin{tabular}{llll}
% \hline \hline
% Dimension & Level-set function & Outer Normal & Mean Curvature \\ \hline \hline
% \\[-0.5em]
%  $d=2$ & $\Phi(y) = y_2 - \frac{y_1^2}{a}$ & $\nu(y) = \frac{(2y_1/a,-1)^\top}{\sqrt{1+ 4y_1^2/a^2}}$ & $\kappa(y)  = \frac{2/a}{(1+ 4y_1^2/a^2)^{3/2}}$\\[1.5em]
%   $d=3$ &  $\Phi(y) = y_3 - \frac{y_1^2}{a} +  \frac{y_2^2}{b}$ 
%   & $\nu(y)= \frac{\left(\frac{2y_1}{a},\frac{2y_1}{b},-1\right)^\top}{\left(1+ \frac{4y_1^2}{a^2} +  \frac{4y_2^2}{b^2}\right)^{1/2}}$ & $\kappa(y) = \frac{\frac{4y_1^2}{a} +  \frac{4y_2^2}{b} + a + b}{ab\left(1+ \frac{4y_1^2}{a^2} +  \frac{4y_2^2}{b^2}\right)^{3/2}}$\\[1.5em]
%  \hline
% \end{tabular}
% \caption{Parabolas.}

% \label{tab:parabolas}
% \end{center}
% \end{table}
 
\begin{figure}[H]
\caption{Estimated  curvature (left panels) and relative error (right panels) for a parabola $(d=2)$ with parameter $a = 2$. }
\vspace{-2mm}

\begin{subfigure}[b]{0.49\textwidth}
    \centering
     \caption{Curvature} \includegraphics[height=1.7in,width=2.2in]{Figures/Curvature fit 2D.pdf}
    \label{fig:curvParaboloid1}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \caption{Relative error} \includegraphics[height=1.7in,width=2.2in]{Figures/Curvature error 2D.pdf}
    \label{fig::errorParaboloid1}
\end{subfigure}

\label{fig:curvParabol2D}
\end{figure}

\begin{figure}[H]
\caption{Estimated mean curvature (left panels) and relative error (right panels) for a paraboloid $(d=3)$ with parameters $(a,b) = (1,2)$ (top panels) and $(a,b) = (-1,2)$ (bottom panels). }
\vspace{-2mm}

\begin{subfigure}[b]{0.49\textwidth}
    \centering
     \caption{Mean Curvature, $(a,b) = (1,2)$} \includegraphics[height=1.7in,width=2.2in]{Figures/Curvature, a = 1.0, b = 2.0.pdf}
    \label{fig:curvParaboloid1}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \caption{Relative error, $(a,b) = (1,2)$} \includegraphics[height=1.7in,width=2.2in]{Figures/Curvature Error, a = 1.0, b = 2.0.pdf}
    \label{fig::errorParaboloid1}
\end{subfigure}
\vspace{3mm}

\begin{subfigure}[b]{0.49\textwidth}
    \centering
     \caption{Mean Curvature, $(a,b) = (-1,2)$} \includegraphics[height=1.7in,width=2.2in]{Figures/Curvature, a = -1.0, b = 2.0.pdf}
    \label{fig:curvParaboloid2}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \caption{Relative error, $(a,b) = (-1,2)$} \includegraphics[height=1.7in,width=2.2in]{Figures/Curvature Error, a = -1.0, b = 2.0.pdf}
    \label{fig::errorParaboloid2}
\end{subfigure}

\label{fig:curvParabol3D}
\end{figure}

% \begin{figure}[H]
% \caption{Estimated mean curvature (left panels) and relative error (right panels) for a hyperbolic paraboloid $(d=3)$ with parameteres $(a,b) = (-1,2)$.  }
% \vspace{-2mm}


% \label{fig:curvHyperParabol}
% \end{figure}

